Fixing Bug Reporting for Mobile and GUI-Based Applications

Smartphones and tablets have established themselves as mainstays in the modern computing landscape. It is conceivable that in the near future such devices may supplant laptops and desktops, becoming many users primary means of carrying out typical computer assisted tasks. In turn, this means that mobile applications will continue on a trajectory to becoming more complex, and the primary focus of millions of developers worldwide. In order to properly create and maintain these apps developers will need support, especially with regard to the prompt confirmation and resolution of bug reports. Unfortunately, current issue tracking systems typically only implement collection of coarse grained natural language descriptions, and lack features to facilitate reporters including important information in their reports. This illustrates the lexical information gap that exists in current bug reporting systems for mobile and GUI-based apps. This paper outlines promising preliminary work towards addressing this problem and proposes a comprehensive research program which aims to implement new bug reporting mechanisms and examine the impact that they might have on related software maintenance tasks.

==> ack.tex <==
This work is supported in part by the NSF CCF-1218129 and NSF CCF-1253837 grants.  Any opinions, findings, and conclusions expressed herein are the authors' and do not necessarily reflect those of the sponsors.   We would like to thank Martin White for his invaluable guidance at the outset of this project and the anonymous reviewers for their insightful comments which greatly improved this paper.

==> approach.tex <==

    %\Fusionsp's \textit{Analyze} $\rightarrow$ \textit{Generate} workflow corresponds to two major phases. In the \textit{Analysis Phase} \Fusionsp collects information related to the GUI components and event flow of an app through a combination of static and dynamic analysis.  Then in the \textit{Report Generation Phase} \Fusionsp takes advantage of the GUI centric nature of mobile apps to both auto-complete the steps to reproduce the bug and augment each step with contextual application information.  The overall design of \Fusionsp can be seen in Figure \ref{Design}.  We encourage readers to view videos of our tool in use, complete with commentary, available in our replication package outlined in Section \ref{sec:rep-pack} and online at \cite{appendix}.
    
\Fusions current target user base consists of two major groups: \textit{mobile application developers} and \textit{testers} or \textit{beta} users.  As such there are two user scenarios for the tool's use.  From a developer's perspective the workflow is purposefully simple; the only action required is the submission of an \texttt{.apk} of the latest build of the application for which they want to enable bug reporting.  Once this file is submitted, \Fusions automated program analysis techniques extract the information necessary to facilitate process of creating a bug from the reporters end.  Once reports are filled out, developers can access them through a web portal.  From a reporter's perspective, they construct a report using a web interface.  After selecting the application for which they would like to report a bug, the reporter enters a brief description and contextual information about the bug (e.g. device used, screen orientation).  They then use a series of auto-filled combo boxes to construct reproduction steps, including screenshots.

%-------------------------------------------------------------------------
\subsection{FUSION Architecture}
 
Fusion's architecture can be seen in Figure \ref{Design}. First, \Fusionsp collects information related to the GUI components and event flow of an app using the \textit{Static Application Analyzer} and the \textit{Dynamic Analysis Engine}.  Then the tool leverages the information collected during the analysis to facilitate a reporter constructing a detailed bug report with reproduction steps, and screenshots.
    The static and dynamic analyses must be performed before each version of an app is released for testing or before it is published to end users.  Both program analysis components store their extracted data in the \Fusionsp database (Fig. \ref{Design} - \circled{3}).
    
\subsubsection{Static Analysis}
    
    The goal of the \emph{Static App Analyzer} (Fig. \ref{Design} - \circled{1})
   is to extract all of the GUI components and associated information from the app source code.   For each GUI component, the \emph{Primer} extracts: (i) possible actions on that component, (ii) type of the component (e.g., Button, Spinner), (iii) activities the component is contained within, and (iv) class files where the component is instantiated.  Thus, this results in a universe of possible components within the domain of the application, and establishes traceability links connecting GUI components that reporters operate upon to code specific information such as the class or activity they are located within.  
    
    The \emph{Static App Analyzer} utilizes several tools to extract the information outlined above. First it uses the  {\tt dex2jar}\cite{dex2jar} and  {\tt jd-cmd} \cite{jd-cmd}  tools for decompilation; then, it converts the source files to an XML-based representation using {\tt srcML} \cite{srcml}. We also use {\tt apktool} \cite{apktool} to extract the resource files from the app's APK.  The {\tt id}s and types of GUI components were extracted from the xml files located in the app's resource folders (\textit{i.e.},  {\tt /res/layout} and  {\tt /res/menu} of the decompiled application or src).  Using the {\tt srcML} representation of the source code, we are able to parse and link the GUI-component information to extracted app source files.  
    
\subsubsection{Dynamic Analysis}

The \emph{Dynamic Analysis Engine} (Fig. \ref{Design} - \circled{2}) is used to glean dynamic contextual information and enhance the database with both run-time GUI and application event-flow information. The goal of the \emph{Engine} is to explore an app in a systematic manner, ripping and extracting run-time information related to the GUI components during execution including: (i) the text associated with different GUI components (e.g., the ``Send'' text on a button to send an email message), (ii) whether the GUI component triggers a transition to a different activity, (iii) the action performed on the GUI component during systematic execution, (iv) full screen-shots before and after each action is performed, (v) the location of the GUI component object on the test device's screen, (vi) the current activity and window of each step, (vii) screen-shots of the specific GUI component, and (viii) the object index of the GUI component (to allow for differentiation between different instantiations of the same GUI component on one screen). 

\begin{figure}[tb]
\centering
\includegraphics[width=\linewidth]{img/FUSION-Tool-Demo-Design.pdf}
\vspace{-0.3cm}
\caption{\Fusionsp Architecture}
\label{Design}
\end{figure}
 
    The \emph{Engine} performs this systematic exploration of the app using the {\tt UIAutomator} \cite{uiautomator} framework included in the Android SDK.  This systematic execution of the app is similar to existing approaches in GUI ripping \cite{Amalfitano:ASE2012,Azim:OOPSLA2013,Machiry:FSE2013}. Using the {\tt UIAutomator} framework allows us to capture cases that are not captured in previous tools such as pop-up menus that exist within menus, internal windows, and the onscreen keyboard.  To effectively explore the application we implemented our own version of a systematic depth-first search (DFS) algorithm for application traversal that performs click events on all the clickable components in the GUI hierarchy reachable using the DFS heuristic.
      
    %During the ripping, before each step is executed on the GUI, the \emph{Engine} calls {\tt UIAutomator} 
    %\DENYS{please be consistent in highlighting all the names of the tools consistently}
    %\KEVIN{Fixed the highlighting of the names}
    % subroutines to extract the contextual information outlined above regarding each currently displayed GUI component.  We then execute the action associated with each GUI component in a depth-first manner on the current screen. Our current implementation of DFS only handles the click/tap action; however, as this is the most common action, it is still able to explore a significant amount of an application's functionality.  
     
     %In the DFS algorithm, if a link is clicked that would normally transition to a screen in an external activity (e.g., clicking a web link that would launch the Chrome web browser app), we execute a \textit{back} command in order to stay within the current app.  If the DFS exploration exits the app to the home screen of the device/emulator for any reason, we simply re-launch the app and  continue the GUI traversal.  During the DFS exploration, the \emph{Engine} captures every activity transition that occurs after each action is performed (e.g., whether or not a new activity is started/resumed after an action to launch a menu).  This allows \Fusionsp to build a model of the app execution that we will later use to help track a reporter's relative position in the app when they are using the system to record the steps to reproduce a bug.  
%-------------------------------------------------------------------------
\subsection{Reporting Bugs with FUSION}  
       
                During the \emph{Report Generation Phase}, \Fusionsp aids the reporter in constructing the steps needed to recreate a bug by making suggestions based upon the ``potential" GUI state reached by the declared steps.  This means for each step $s$, \Fusionsp infers --- online --- the GUI state $GUI_s$ in which the target app should be by taking into account the history of steps.   For each step, \Fusionsp verifies that the suggestion made to the reporter is correct by presenting the reporter with contextually relevant screen-shots, where the reporter selects the screen-shot corresponding to the current action the reporter wants to describe. 
                
                % The Report Generator component of \Fusionsp can be separated into two logical components, (i) the UI-centric front end and (ii) the back-end suggestion algorithm with database interface.  We will now describe both of these components in detail. 
                
                %\MARIO{The focus of the section should be the approach and not the tool. You are providing implementation details that are irrelevant. So, I commented the sentence talking about implementation details. I also reorganized the subsections to explain first the underlying approach and then show the \Fusionsp UI}
    		%\KEVIN{CORRECTION: Good point Mario, I have cleaned up the section to reflect these changes in a more coherent manner}
		
\subsubsection{Report Generator User Interface}

%\MARIO{Kevin, please highlight in Figure 2 the subsections in the \Fusionsp UI and use that Figure to explain the UI in section 3.2.1}
\begin{figure}[t]
\centering
\includegraphics[width=\linewidth]{img/fusion-report-interface-final.pdf}
\vspace{-0.5cm}
\caption{\Fusionsp Reporting Interface}
\label{front_end}
\end{figure}

    After first selecting the app to report an issue for, a reporter interacts with \Fusionsp by filling in some identifying information (i.e., name, device, title) and a brief textual description of the bug in the top half of the UI.  Next, the reporter inputs the steps to reproduce the bug using the auto-completion boxes in a step-wise manner, starting from the initial screen of a cold app launch\footnote{Cold-start means the first step is executed on the first window and screen displayed directly after the app is launched.}, and proceeds until the list of steps to reproduce the bug is exhausted.  According to the various fields in Figure \ref{front_end}, the reporter would first fill in their (i) \textit{name} (Field 1), (ii) \textit{device} (Field 2), (iii) \textit{screen orientation} (Field 3), (iv) a \textit{bug report title} (Field 4), and (v) a \textit{brief description of the bug} (Field 5). 
     
     The first drop down list (see Figure \ref{front_end} - Field 6) corresponds to the possible actions a user can perform at a given point in app execution.  For example, let's say the reporter selects \textit{click} as the first action in the sequence of steps as shown in Figure \ref{front_end}. The possible actions considered in \Fusionsp  are \textit{click(tap), long-click(long-touch), type}, and \textit{swipe}.  The \textit{type} action corresponds to a user entering information from the device keyboard.  When the reporter selects the \textit{type} option, we also present them with a text box to collect the information she typed in the Android app.

	The second dropdown list (see Figure \ref{front_end} - outlined in blue) corresponds to the component associated with the action in the step. \Fusionsp presents the following information, which can also be seen in Figure \ref{front_end}: (i) \textit{Component Type}: this is the type of component that is being operated upon, e.g., button, spinner, checkbox,  (ii) \textit{Component Text}: the text associated with or located on the component, (iii) \textit{Relative Location}: the relative location of the component on the screen according to the parameters in Figure \ref{example_screenshot}, and (iv) \textit{Component Image}: an in-situ (i.e., embedded in the dropdown list) image of the instance of the component.  The relative location is displayed here to make it easier for reporters to reason about the on-screen location, rather than reasoning about pixel values.  In our running example, \Fusionsp will populate the component dropdown list with all of the clickable components in the \texttt{main} Activity since this is the first step and the selected action was \textit{click}.  
	    
   \Fusion uses two techniques to handle instances of seemingly identical GUI-component appearing on the same screen. \textit{First}, it differentiates each duplicate component in the list through specifying text ``Option \#''.  \textit{Second} \Fusionsp attempts to confirm the component entered by the reporter at each step by fetching screen-shots from the \Fusionsp database representing the entire device screen (e.g. Figure \ref{example_screenshot}) .
    
    \begin{figure}[t]
\centering
\includegraphics[width=\linewidth]{img/example_screenshot_combined.pdf}
\vspace{-0.8cm}
\caption{Relative Location Enumeration and Example Augmented Screenshot}
\label{example_screenshot}
\end{figure}
    
     After the reporter makes selections from the drop-down lists, they have an opportunity to enter additional information for each step (e.g., a button had an unexpected behavior) in a natural language text entry field.  For instance, the reporter might indicate that after pressing the ``OK" button the pop-up window took longer than expected to disappear.  
   
   \subsubsection{Report Generator Auto-Completion Engine}
 
 The \emph{Auto-Completion Engine} of the web-based report generator (Figure \ref{Design}-\circled{4}) uses the information collected up-front during the \textit{Analysis Phase}. When \Fusionsp suggests completions for the drop-down menus, it queries the database for the corresponding state of the app event flow and suggests information based on the past steps that the reporter has entered.  Since we always assume a ``cold'' application start, the \emph{Auto-Completion Engine} starts the reproduction steps entry process from the app's \texttt{main} Activity.  We then track the reporter's progress through the app using predictive measures based on past steps.  
 
 	%The \emph{Auto-Completion Engine} operates on application steps using several different pieces of information as input.  It models the reporter's reproduction steps as an ordered stream of steps $S$ where each individual step $s_i$ may be either empty or full.  Each step can be modeled as a five-tuple consisting of \textit{\{step\_num, action, comp\_name, activity, history\}}.  The \textit{action} is the gesture provided by the reporter in the first drop-down menu.  The \textit{component\_name} is the individual component name as reported by the {\tt UIautomator} interface during the Engine phase.  The \textit{activity} is the Android screen the component is found on.  The \textit{history} is the history of steps preceding the current step.  The auto-completion engine predicts the suggestion information using the decision tree logic which can be seen in Figure \ref{decision_tree}.  
	
	\Fusionsp presents components to the reporter at the granularity of activities or application screens.  During the suggestion process, \Fusionsp looks back through the history of the past few steps and looks for possible transitions from the previous steps to future steps depending on the components interacted with.  If \Fusionsp is unable to capture the last few steps from the reporter due to the incomplete application execution model mentioned earlier, then \Fusionsp presents the possibilities from all known screens of the application. In our running example, let's consider the reporter moving on to report the second reproduction step.  Due to the limited nature of the DFS heuristic used by the \textit{Dynamic Analysis Engine}, there may be action-Gui-Component pairs that are not available in the auto-filled combo boxes.  To handle these cases gracefully, we allow the reporter to select a special option when they cannot find the component they interacted with in the auto-complete drop-down list.  In these cases the reporter would manually fill in (i) the type of the component, (ii) any text associated with the GUI-component and (iii) the relative location of the GUI-component as denoted in Figure \ref{example_screenshot}.
		 
   \begin{figure}[t]
\centering
\includegraphics[width=0.95\linewidth]{img/report.pdf}
\vspace{-0.4cm}
\caption{Example \Fusionsp Bug Report}
\label{report}
\end{figure}  
   
%\subsubsection{Handling \Fusionsp's Application Model Gaps}
    
    %Because DFS-based exploration is not exhaustive, there may be gaps in \Fusionsp's database of possible app screens (e.g., a dynamically generated component that triggers an activity transition was not acted upon). Due to this, a reporter may not find the appropriate suggestion in the drop-down list.  To handle these cases gracefully, we allow the reporter to select a special option when they cannot find the component they interacted with in the auto-complete drop-down list. In our running example, let's say the reporter wishes to indicate that they clicked the button labeled ``Open Document," but the option is not available in the auto-complete component drop-down list.  In this case the reporter would select the ``Not in this list...'' option and manually fill in  (i) the type of the component (to limit con\Fusionsp, we present this option as a drop-down box auto-completed with only the GUI-component types that exist in the application, as extracted by the \emph{Primer}, in our case the user would choose ``Button"), (ii) any text associated with the GUI-component (in this case ``Open Document") and (iii) the relative location of the GUI-component as denoted in Figure \ref{example_screenshot} (in this case ``Top Center").

\subsubsection{Viewing FUSION Reports}

      The \emph{Auto Completion Engine} saves each step to the database as reporters complete bug reports.  Once a reporter finishes filling out the steps and completes the data entry process, a screen containing the final report, with an automatically assigned unique ID, is presented to the reporter and saved to the database for a developer to view later (see Figure \ref{report} for an example report). 

       The Report presents information to developers in three major sections: First, preliminary information including the report title, device, and short description (shown in Figure \ref{report} in blue).  Second, a list of the Steps with the following information regarding each step is displayed (highlighted in blue in Figure \ref{report}): (i) The action for each step, (ii) the type of a component, (iii) the relative location of the component, (iv) the activity Java class where the component is instantiated in the source code, and (v) the component specific screenshot.  Third, a list of full screen-shots corresponding to each step is presented at the bottom of the page so the developer can trace the steps through each application screen (this section is highlighted in green in Figure \ref{report}). 

    

    
     

==> evaluation.tex <==
To evaluate \Fusionsp (See full details in \cite{Moran:FSE2015}) we investigated its ease of use, as well as the reproducibility of the \Fusionsp reports compared to reports created using Google Code Issue Tracker (GCIT).  First, in the \textit{bug-creation study} we recruited eight students (four undergraduate or \textit{non-experts} and four graduate or \textit{experts}) to construct bug reports using \Fusionsp and GCIT --- as a representative of traditional bug tracking systems--- for 15 real-world world bugs for 14 open-source apps from F-Droid \cite{fdroid}.  We collected survey responses from these participants regarding the ease of use and user preferences of each tool.  Next, in the \textit{bug-reproduction study} we evaluated the reproducibility of the \Fusionsp and GCIT reports generated by the first group of participants. These reports (120 for each type) and the original bug reports extracted from the respective app issue trackers were evaluated by a new set of 20 graduate student participants through attempted bug reproduction on physical devices.  The results of this study indicate that  developers using \Fusion reports are able to reproduce more reports compared to traditional bug tracking systems such as the GCIT.  

==> macro.tex <==


\usepackage{amssymb}
\usepackage{ifthen}

\makeatletter

% this  is a easy way to add and highlight new text  ...
% just comment in/out the \tnew macro ..

\newcommand{\tnew}[1]{{\bf { #1 }} }
%\newcommand{\tnew}[1]{{ { #1 }} }

% math and theorem definition

\newcommand{\ndef}{\stackrel{\rm def}{=}}

% this is used for draft only

%\renewcommand{\baselinestretch}{2}

% just to number pages in the draft

\pagenumbering{arabic}

% nothing i.e., no-numbering final and camera ready

%\pagestyle{empty}


\newboolean{showcomments}


\setboolean{showcomments}{true}

\ifthenelse{\boolean{showcomments}}
  {\newcommand{\nb}[2]{
    \fbox{\bfseries\sffamily\scriptsize#1}
    {\sf\small$\blacktriangleright$\textit{#2}$\blacktriangleleft$}
   }
   \newcommand{\cvsversion}{\emph{\scriptsize$-$Id: macro.tex,v 1.9 2005/12/09 22:38:33 giulio Exp $}}
  }
  {\newcommand{\nb}[2]{}
   \newcommand{\cvsversion}{}
  }



\newcommand\MARTY[1]{\nb{MARTY}{#1}}
\newcommand\KEVIN[1]{\nb{KEVIN}{#1}}
\newcommand\DENYS[1]{\nb{DENYS}{#1}}
\newcommand\MARIO[1]{\nb{MARIO}{#1}}
\newcommand\CARLOS[1]{\nb{CARLOS}{#1}}

\newcommand\NEW[1]{\nb{NEW}{#1}}





